A Unified Framework for Adversarial Attack and Defense in Constrained Feature Space

The generation of feasible adversarial examples is necessary for properly assessing models that work in constrained feature space. However, it remains a challenging task to enforce constraints into attacks that were designed for computer vision. We propose a unified framework to generate feasible adversarial examples that satisfy given domain constraints. Our framework can handle both linear and non-linear constraints. We instantiate our framework into two algorithms: a gradient-based attack that introduces constraints in the loss function to maximize, and a multi-objective search algorithm that aims for misclassification, perturbation minimization, and constraint satisfaction. We show that our approach is effective in four different domains, with a success rate of up to 100%, where state-of-the-art attacks fail to generate a single feasible example. In addition to adversarial retraining, we propose to introduce engineered non-convex constraints to improve model adversarial robustness. We demonstrate that this new defense is as effective as adversarial retraining. Our framework forms the starting point for research on constrained adversarial attacks and provides relevant baselines and datasets that future research can exploit.

==> 2-related_work.tex <==

\section{Related work}
\label{sec:related}

\subsection{Genetic algorithm for adversarial attacks}

Genetic algorithms are considered as black-box  attack candidates by researchers in many domains. In the category of natural language processing, there exist several attacks using genetic algorithms as a search method. \cite{alzantot2018generating} were the first to use GA to replace words in a sentence with their synonyms to  generate adversarial examples. that preserve semantics and syntax. Synonyms are assumed to preserve the syntax and semantics, therefore they do not use any constraint evaluation like in \moeva{}. These attacks are specific to text and can not be used in other domains. 
%At the same time, the scope of \moeva{} does not cover adversarial attacks in text as it considers explicit constraints between features. In parallel,~\cite{alzantot2018did} had demonstrated the first kind of adversarial attack against a speech recognition model. Similarly, they use a genetic algorithm to add noise to only the least significant bits of a random subset of audio samples. However, there was no study to show if a person could detect the fact that the audio file was tampered. 
The other adaptions of GA appear in~\cite{xu2016automatically}  where the authors modify malicious PDF samples to evade binary malware classifiers. Similarly, in~\cite{kucuk2020deceiving} the authors used a genetic algorithm to evade three multi-class Portable Executable (PE) malware classifiers on targeted attacks. For both PDF and PE attacks, the authors had to check the validity of the generated examples in problem space by passing them through a checker. The advantage of \moeva{} is that it ensures feasibility by including a constraint evaluation process. This avoids the need to reconstruct samples in the problem space and  evaluating them for feasibility. 


% imilar to images, they try to minimize the number of modified words between the original and adversarial examples.  and they need to satisfy  semantic coherence constraints.

% An improved version of Alzantot et al. attack appeared in~\cite{wang2019natural}. It overcomes the limitation of the original attack that substitutes words at the same position only once, avoiding the local minimum. Additional changes are made to the structure of the original algorithm, including the operators for crossover and mutation.
% Both the above attacks work on text data 

\subsection{Adversarial attacks for constrained domains}
 In the constrained adversarial attacks literature, most of the studies upgrade existing attacks to support some constraints and only a few propose new algorithms tailored  to each domain specifically. One of these novel methods for crafting adversarial attacks that respect domain constraints was proposed by~\cite{kulynych2018evading}. The authors use a graphical framework where each edge represents a feasible transformation%, with its weight representing the transformation cost. The nodes of the graph are the transformed examples. Despite the idea being innovative, the 
 .The downside of this method is that it works only with linear models, and it comes with high computation cost. ~\cite{chernikova2019fence} builds an iterative gradient-based adversarial attack that considers groups of feature families. %At each iteration, the feature of maximum gradient and its family, is chosen for modification. The modifications that do not respect the constraints are updated until they enter a feasible region. 
 The implementation provided by the authors is closely related to the botnet domain, therefore it can not be re-used in new domains.  ~\cite{li2020conaml} considers simple linear constraints for cyber-physical systems. They generate practical examples using a best-effort search algorithm. However, the solution is not scalable to practical applications that have more complex non-linear constraints. Our unified framework overcomes the barriers of domain adaptation by providing an easy language to define both linear and non-linear constraints. 

Other researchers 
%have preferred  to 
tune existing attacks to support constraints. ~\cite{sheatsley2020adversarial} extends the traditional JSMA algorithm to support constraints resolution. They  use the concept of a primary feature in a group of interdependent features. Meanwhile, Tian et al.~\cite{tian2020exploring} introduced C-IFGSM an updated version of FGSM that considers feature correlations. %They embed the correlations into a constraint matrix which is  used to calculate the Hadamard product with the sign of the gradient in order to determine the direction and magnitude of the update. 
~\cite{teuffenbach2020subverting} crafted constrained adversarial examples for NIDS by extending the optimization function in Carlini and Wagner attack. They group ﬂow-based features by their modification feasibility  and assign weights to each group based on the level of difficulty of the modification.  %The authors in~\cite{erdemir2021adversarial} introduce non-uniform perturbation in PGD attack to enable adversarial retraining with more realistic examples. They use Pearson’s correlation coefficient, Shapley values, and masking to build a matrix that constrains the direction and magnitude  of change similarly to~\cite{tian2020exploring}. 
All the %existing 
attacks above are upgraded to handle simple and general constraints, but do not deal with more complex domain-specific constraints. Therefore, the samples they generate are more restricted but not totally feasible. 

~\cite{ghamizi2020search} proposed a black-box, genetic-based approach  to generate  constrained adversarial examples for an industrial credit scoring system. This work is the closest to one of the attacks we propose.  Contrary to them, for \moeva{} we are using a multi-objective function that is not case-specific and needs neither parameter tuning nor domain expert knowledge to work. Our framework is more general and can be applied to multiple use cases without fine-tuning.

% However, their fitness function considers each objective separately and assigns weights to their importance.

